Design and characterization of a ground-based absolute polarization calibrator for use with polarization sensitive CMB experiments

We present the design and characterization of a ground-based absolute polarization angle calibrator accurate to better than 0.1 degrees for use with polarization sensitive cosmic microwave background (CMB) experiments. The calibrator's accuracy requirement is driven by the need to reduce upper limits on cosmic polarization rotation, which is expected to be zero in a large class of cosmological models. Cosmic polarization effects such as cosmic birefringence and primordial magnetic fields can generate spurious B-modes that result in non-zero CMB TB and EB correlations that are degenerate with a misalignment of detector orientation. Common polarized astrophysical sources used for absolute polarization angle calibration have not been characterized to better than 0.5 degrees. Higher accuracy can be achieved through self-calibration methods, however these are subject to astrophysical foreground contamination and inherently assume the absence of effects like cosmic polarization rotation. The deficiencies in these two calibration methods highlight the need for a well characterized polarized source. The calibrator we present utilizes a 76 GHz Gunn oscillator coupled to a frequency doubler, pyramidal horn antenna, and co-rotating wire-grid polarizer. We use an accurate bubble level in combination with four precision-grade aluminum planes located within the enclosure to calibrate the source's linear polarization plane with respect to the local gravity vector to better than the 0.1 degree goal. In 2017 the calibrator was deployed for an engineering test run on the POLARBEAR CMB experiment located in Chile's Atacama Desert and is being upgraded for calibration of the POLARBEAR-2b receiver in 2018. In the following work we present a detailed overview of the calibrator design, systematic control, characterization, deployment, and plans for future CMB experiment absolute polarization calibration.

==> conclusions.tex <==
\section{CONCLUSIONS}
\label{sec:conclusions}

The ground-based absolute detector polarization angle calibrator for use with CMB experiments discussed in this paper utilizes a rotating polarized microwave source with co-rotating polarizing wire grid and was designed to be compact, robust to harsh environments, and accurate to better than 0.1$^\circ$ in order to reduce upper limits on the CMB TB and EB correlations and allow for the search of evidence of CPR effects such as cosmic birefringence and PMFs. The calibrator was proven in the laboratory to a consistency within the 0.1$^\circ$ requirement. From its deployment in March 2017 on the POLARBEAR telescope, the calibrator was proven to successfully couple to POLARBEAR detectors, the control and analysis procedure was verified, and detector response was observed to exhibit the expected behavior when rotating the calibrator source. The successful laboratory characterization combined with the successful coupling of the calibrator to the POLARBEAR telescope proves that this type of calibrator design can reach the 0.1$^\circ$ accuracy requirement and is being improved to perform calibration of future CMB experiments. The improved calibrator design is expected to be built and characterized in the laboratory by the end of 2018 using the POLARBEAR-2b receiver and will be compatible with future CMB experiments such as the Simons Array and the Simons Observatory.
